A Survey of Community Search Over Big Graphs

With the rapid development of information technologies, various big graphs are prevalent in many real applications (e.g., social media and knowledge bases). An important component of these graphs is the network community. Essentially, a community is a group of vertices which are densely connected internally. Community retrieval can be used in many real applications, such as event organization, friend recommendation, and so on. Consequently, how to efficiently find high-quality communities from big graphs is an important research topic in the era of big data. Recently a large group of research works, called community search, have been proposed. They aim to provide efficient solutions for searching high-quality communities from large networks in real-time. Nevertheless, these works focus on different types of graphs and formulate communities in different manners, and thus it is desirable to have a comprehensive review of these works. In this survey, we conduct a thorough review of existing community search works. Moreover, we analyze and compare the quality of communities under their models, and the performance of different solutions. Furthermore, we point out new research directions. This survey does not only help researchers to have a better understanding of existing community search solutions, but also provides practitioners a better judgment on choosing the proper solutions.

==> CD.tex <==
\subsection{Community Detection}
\label{sec:CD}

Below, we review representative CD studies on undirected graphs, directed graphs, and attributed graphs.

\subsubsection{Undirected Graphs}
\label{sec:CDSimple}

A large number of studies aim to detect communities from simple graphs, and we can classify these studies based on the techniques they use. Some representative classes are as follows, to name a few:
\begin{enumerate}
  \item community quality optimization-based methods (e.g., modularity \cite{newman2004fast});
  \item clustering methods (e.g., $k$-means \cite{tang2009scalable}, spectral clustering \cite{von2007tutorial});
  \item graph partitioning methods (e.g., Metis \cite{karypis1995metis});
  \item embedding-based methods (e.g., DeepWalk \cite{perozzi2014deepwalk}, \cite{li2018community});
  \item random walk-based methods (e.g., \cite{pons2005computing});
  \item label propagation-based methods (e.g., \cite{gregory2010finding});
  \item information diffusion-based methods (e.g., \cite{hajibagheri2012community});
  \item statistic inference-based models (e.g., \cite{hastings2006community});
  \item deep learning-based methods (e.g., \cite{Yang:2016});
  \item centrality-based methods (e.g., \cite{community-phy2004});
  \item locality sensitive hashing-based methods (e.g., \cite{macropol2010scalable});
  \item physics-based methods (e.g., Potts low \cite{wu1982potts});
  \item local metric-based methods (e.g., $k$-plex \cite{conte2018d2k});
  \item multi-commodity flow-based methods (e.g., \cite{leighton1988approximate});
  \item hybrid-based methods (e.g., \cite{henderson2010hcdf}).
\end{enumerate}

For a detailed survey of CD, please refer to the following survey and empirical evaluation papers:
\cite{CD:Survey:2009,Yang2010,community-phy2010,papadopoulos2012community,danon2005comparing,gulbahce2008art,CD:Survey:2011,CD:Survey:2011a,CD:Survey:2013,CD:Survey:2017,CD:Survey:2014-overlap,CD:Survey:2015-multilayer,CD:Survey:2018-dynamic,CD:Survey:2010-compare,CD:Survey:2014-evaluate,CD:Survey:2015-truth}.
Although these CD solutions are able to discover communities from networks, they may not well satisfy the desirable factors of CS on big graphs as we discuss in Section \ref{sec:intro}, because most of them often use a global predefined criterion for generating communities and cannot find communities in an online manner.


\subsubsection{Directed Graphs}
\label{sec:CDDirected}

In recent years, a number of studies have investigated CD on directed graphs. Here are some representative studies, to name a few.
In~\cite{prl2008}, Leicht et al. extended the concept of modularity maximization~\cite{newman2004fast}, which was originally designed for undirected graphs, for detecting community structure in directed networks that makes explicit use of information contained in edge directions. In \cite{flake2000}, Flake et al. identified communities from websites network, which can be considered as directed graphs.
In~\cite{CDBenchmark}, Lancichinetti et al. introduced new benchmark graphs to test CD methods on directed
networks.
In~\cite{pre2010}, Kim et al. also proposed a new modularity metric for CD on directed networks.
In~\cite{sdm2010}, Yang et al. developed a new stochastic block model for CD on directed networks.
In~\cite{yang2014detecting}, Yang et al. presented algorithms for detecting communities from both directed and undirected networks.
Ning et al. \cite{ning2016local} studied local community extraction in directed networks.
A recent survey can be found in~\cite{CDSurvey}.

\subsubsection{Keyword-Based Attributed Graphs}
\label{sec:CDKeyword}

To identify communities from keyword-based attributed graphs, recent works~\cite{attr-vldb2009,SDM2013,WSDM2013,cheng2012clustering,huang2012semi,attr-www2013} often use clustering techniques. Zhou et al. \cite{attr-vldb2009} computed vertices' pairwise similarities using both links and keywords, and then clustered the graph.
Subbian et al. \cite{SDM2013} explored noisy labeled information of graph vertices for finding communities.
Qi et al. \cite{WSDM2013} dynamically maintained communities of moving objects using their trajectories.
Ruan et al.~\cite{attr-www2013} developed a method {\tt CODICIL}, which augments the original graph by creating new edges based on content similarity, and then performs clustering on the new graph. Huang et al.~\cite{huang2016attributed} investigate community detection and community search in attributed networks, respectively in terms of global network-wide analysis and ego-centric personalized analysis aspects. 

Another common approach is based on topic models. In~\cite{attr-topic-kdd2008,attr-topic-icml2009}, the {\tt Link-PLSA-LDA} and {\tt Topic-Link LDA} models jointly model vertices' content and links based on the {\tt LDA} model. In~\cite{attr-topic-sigmod2012}, the attributed graph is clustered based on probabilistic inference. In~\cite{attr-topic-www2012}, the topics, interaction types, and the social connections are considered for discovering communities. {\tt CESNA}~\cite{yang2013community} detects overlapping communities by assuming communities ``generate'' both the link and content. A discriminative approach~\cite{attr-kdd2009} has also been considered for community detection.
However, computing pairwise similarity among vertices is very costly, and thus they are questionable for performing online CS queries.



\subsubsection{Location-Based Attributed Graphs}
\label{sec:CDLocation}

The problem of CD on location-based attributed graphs (or geo-social networks) \cite{barthelemy2011} has been extensively studied \cite{girvan2002,guo2008,pnas2011,KDD2013,IJGIS2015}. In \cite{girvan2002}, Girvan et al. introduced the geo-community, which is a graph of intensely connected vertices being loosely connected with others, but it is more compact in space.
Guo et al.~\cite{guo2008} proposed the average linkage (ALK) measure for clustering objects in spatially constrained graphs.
In~\cite{pnas2011}, Expert et al. uncovered communities from spatial graphs based on modularity maximization.
In~\cite{KDD2013}, Shakarian et al. used a variant of Newman-Girvan modularity to mine the geographically dispersed communities.
In~\cite{IJGIS2015}, Chen et al. proposed a method using modularity maximization for detecting communities from geo-social networks.

\subsubsection{Temporal Graphs}
\label{sec:CDTemporal}

Many recent studies aim to detect communities from temporal graphs. In \cite{zhou2007discovering}, Zhou et al. studied CD over a temporal heterogeneous social network consisting of authors, document content, and the venues.
In \cite{liu2014persistent}, Liu et al. studied persistent community detection for identifying communities that exhibit persistent behavior over time.
In \cite{angadi2015overlapping}, Angadi et al. detected communities from dynamic networks where data arrives as a
stream to find the overlapping vertices in communities.
In \cite{bazzi2016community}, Bazzi et al. investigated the detection of communities in temporal multi-layer networks.
In \cite{ditursi2017local}, DiTursi et al. proposed a filter-and-verify framework for community detection in dynamic networks.
In \cite{kuncheva2017multi}, Kuncheva et al. presented a method by using spectral graph wavelets to detect communities in temporal graphs.
For more related studies, please refer to survey papers \cite{CD:Survey:2018-dynamic,tamimi2015literature}.


==> GKS.tex <==
\subsection{Graph Keyword Search}
\label{sec:GKS}

Generally, graph keyword search \cite{wang2010survey,keyword-yu-2009} aims to find a tree or a subgraph, which contains a set of query keywords, from a large graph $G$. Earlier studies often output a tree structure.
In~\cite{keyword-icde2002}, Bhalotia et al. developed a backward algorithm for finding Steiner trees.
In~\cite{keyword-icde2007}, Ding et al. proposed a dynamic programming algorithm finding Steiner trees.
In~\cite{golenberg2008keyword}, Golenberg et al. presented a novel algorithm which produces Steiner trees with polynomial delay.
In~\cite{keyword-vldb2005}, Kacholia et al. proposed a bidirectional search algorithm, and He et al.~\cite{he2007blinks} improved it by introducing a new index structure.

Recently, some solutions have output subgraphs.
In \cite{keyword-sigmod2008}, Li et al. proposed to find $r$-radius Steiner graphs that contain query keywords.
Qin et al. \cite{keyword-icde2009} proposed to find multi-centered subgraphs that contain query keywords within a given distance. Kargar et al. \cite{keyword-vldb2011} studied the $r$-clique which is a set of vertices that cover query keywords and satisfy the distance constraint.

However, these works are substantially different from CS queries on keyword-based attributed graphs. First, they do not specify query vertices as required by CS queries. Second, the tree or subgraph produced do not guarantee structure cohesiveness. Third, their solutions do not ensure strong keyword cohesiveness.


==> GPM.tex <==
\subsection{Graph Pattern Matching (GPM)}
\label{sec:GPM}
For simple graphs, the problem of GPM is NP-complete \cite{cook1971complexity} and it has been studied extensively under different settings:
(1) in main memory \cite{ullmann1976algorithm,chiba1985arboricity}. For example, Ullmann \cite{ullmann1976algorithm} proposed a backtracking algorithms.
(2) in external memory, Chu et al. \cite{chu2011triangle} and Hu et al. \cite{hu2014efficient} studied triangle counting; in \cite{qiao2017subgraph}, a novel GPM solution based on graph compression is presented.
(3) in distributed platforms, both DFS-style approaches \cite{afrati2013enumerating,park2016pte}and BFS-style approaches \cite{lai2015scalable,lai2016scalable} are developed. The DFS-style approaches avoid intermediate results by using one-round computation, while BFS-style approaches shuffle a large number of intermediate results.

For attributed graphs, there are also many studies. Tong et al. \cite{GPM-KDD2007} studied the use of lines, loops and stars for finding the matched subgraphs; Zou et al. \cite{zou2009distance} developed a novel GPM solution based on distance join;
Fan et al. \cite{GPM-VLDB2010} studied GPM by using bounded simulation; in \cite{GPM-PVLDB2015}, GPM has been studied for finding graph association rules; in \cite{GPM-ICDE2012}, Cheng et al. studied the problem of top-$k$ GPM. Recently, Fang et al. have studied a variant of the GPM problem on spatial databases \cite{Fang:ICDE:SPM,Fang:ICDE:DEMO}, and it aims to find spatial objects that are matched with a given pattern.
However, GPM is different with CS because (1) it often focuses on small patterns, so it cannot generate large communities; and (2) the subgraphs of GPM solutions often do not have guarantee on strong structure cohesiveness. Other related topics include node similarity computation \cite{yu2013more,yu2012space}, keyword search \cite{yuan2017keyword,yuan2013efficient},  and uncertain subgraph search \cite{yua,yuan2012efficient}.


==> cohesive.tex <==
\subsection{Cohesive SubGraph Discovery}
\label{sec:cohesive}

In this section, we review studies on cohesive subgraph discovery. Notice that CD is one kind of cohesive subgraph discovery, but the latter one is more general.

\subsubsection{Simple Graphs}
\label{sec:cohSimple}

For simple graphs, typical cohesive subgraph models are
$k$-core \cite{md1983,kcore2003},
$k$-truss \cite{saito2008extracting,cohen2008trusses,zhang2012extracting},
$k$-clique \cite{kclique,article05clique},
and $k$-ECC \cite{gibbons1985algorithmic,hu2016querying}, as discussed in Section \ref{sec:pre}.
To compute these subgraphs, there are many efficient in-memory algorithms (e.g., $k$-core \cite{kcore2003}, $k$-truss \cite{wang2012truss}, $k$-clique \cite{mauro2018}, and $k$-ECC \cite{zhou2012finding,Chang:SIGMOD:2013,akiba2013linear}).
For graphs that are too large to be kept in memory, there are also some disk-based and parallel algorithms.
For example, in \cite{cheng2011efficient,wen2018efficient}, \cite{wang2012truss,khaouid2015k}, and \cite{cheng2012fast}, disk-based algorithms for computing $k$-core, $k$-truss, and $k$-clique are developed, respectively; in \cite{montresor2013distributed} and \cite{chen2014distributed}, parallel algorithms for computing $k$-core and $k$-truss are proposed, respectively. In addition, to maintain $k$-core and $k$-truss for dynamic graphs, some efficient algorithms are developed in \cite{li2014efficient,sariyuce2016incremental,zhang2017fast} and \cite{zhou2014efficient}, respectively.

Besides, there are many other cohesive subgraph models and the representatives are as follows.
In \cite{seidman1978graph}, Seidman proposed the $k$-plex model (which is introduced in Section~\ref{sec:kclique}).
In \cite{matsuda1999classifying}, Matsuda et al. introduced the concept of quasi-clique model.
In \cite{zhang2018discovering}, Zhang et al. proposed the ($k$, $s$)-core, which considers both user engagement and tie strength.
In \cite{sariyuce2016fast}, the authors proposed the concept of nucleus, which is a generalization of $k$-core and $k$-truss.
In \cite{zhao2012large}, Zhao et al. introduced the mutual-friend subgraph.
In \cite{wang2010triangulation}, Wang et al. proposed the DN-Graphs by considering vertices' common neighbors.
In \cite{Chang:SIGMOD:2013}, Chang et al. studied the problem of enumerating $k$-ECCs in a graph for a given $k$.
In \cite{zhu2018diversified}, Zhu et al. introduced the notion of coherent cores on multi-layer graphs.
In addition, Goldberg et al. \cite{goldberg1984finding} discovered the densest subgraph, Galbrun et al. \cite{Galbrun:2016} studied the top-$k$ densest subgraphs, Tsourakais et al. \cite{tsourakakis2013denser} computed the quasi-clique-based dense subgraphs, and Qin et al. \cite{Qin:2015} proposed and studied the problem of finding top-$k$ locally densest subgraphs.


\subsubsection{Attributed Graphs}
\label{sec:cohAttributed}

For attributed graphs, in addition to CD methods, there are also many studies of finding cohesive subgraphs.
In \cite{denian:2012}, Yang et al. studied the socio-spatial group query which finds a group of users that are cohesively linked and close to the rally point in a geo-social network.
In \cite{Zhang:VLDB:2017}, Zhang et al. studied the problem of finding ($k$, $r$)-cores on attributed graph and for a specific ($k$, $r$)-core, each vertex has at least $k$ neighbors, and the attribute similarity of each pair of vertices is at least $r$.
In \cite{Chen:VLDB:2018}, Chen et al. studied the problem of ($k$, $d$)-MCC (maximum co-located community) search on geo-social network, where a ($k$, $d$)-MCC is a connected $k$-truss and for any two vertices, their distance is at most $d$.
In addition, Wu et al. \cite{wu2015finding} studied the problem of finding the densest connected subgraph from the dual network, which can be considered as an attributed graph.


==> kcliqueLocation.tex <==
\subsection{Location-Based Attributed Graphs}
\label{sec:kcliqueSimple}


==> kcliqueSimple.tex <==
\subsection{Simple Undirected Graphs}
\label{sec:kcoreSimple}


==> ktrussLocation.tex <==
\subsection{Location-Based Attributed Graphs}
\label{sec:ktrussLocation}

